The $s$-weak order and $s$-permutahedra I: combinatorics and lattice structure

This is the first contribution of a sequence of papers introducing the notions of $s$-weak order and $s$-permutahedra, certain discrete objects that are indexed by a sequence of non-negative integers $s$. In this first paper, we concentrate purely on the combinatorics and lattice structure of the $s$-weak order, a partial order on certain decreasing trees which generalizes the classical weak order on permutations. In particular, we show that the $s$-weak order is a semidistributive and congruence uniform lattice, generalizing known results for the classical weak order on permutations. Restricting the $s$-weak order to certain trees gives rise to the $s$-Tamari lattice, a sublattice which generalizes the classical Tamari lattice. We show that the $s$-Tamari lattice can be obtained as a quotient lattice of the $s$-weak order when $s$ has no zeros, and show that the $s$-Tamari lattices (for arbitrary $s$) are isomorphic to the $\nu$-Tamari lattices of Pr\'eville-Ratelle and Viennot. The underlying geometric structure of the $s$-weak order will be studied in a sequel of this paper, where we introduce the notion of $s$-permutahedra.

==> figures/dtrees/F022_1.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=white] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle,fill=red!50] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle,fill=red!50] (d) {$1$}
;}\newcommand{\nodee}{\node[draw,circle,fill=white] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle,fill=white] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodef  \& \nodeg  \&         \\ 
         \& \nodee  \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(c) edge (d) edge (f) edge (g)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}


==> figures/dtrees/F022_2.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=white] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle,fill=red!50] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle,fill=white] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle,fill=red!50] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle,fill=white] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodee  \& \nodeg  \&         \\ 
         \&         \& \nodef  \&         \&         \\
};

\path[ultra thick, red] (e) edge (f)
	(c) edge (d) edge (e) edge (g)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}

==> figures/dtrees/F022_3.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=red!50] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle,fill=white] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle,fill=white] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle,fill=white] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle,fill=red!50] (f) {$1$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodef  \& \nodeh  \\ 
 \nodec  \& \noded  \& \nodee  \& \nodeg  \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d) edge (e)
	(f) edge (g)
	(a) edge (b) edge (f) edge (h);
\end{tikzpicture}}

==> figures/dtrees/F022_inter.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=white] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle,fill=red!50] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle,fill=white] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle,fill=white] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle,fill=white] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodee  \& \nodeg  \&         \\ 
         \&         \& \nodef  \&         \&         \\
};

\path[ultra thick, red] (e) edge (f)
	(c) edge (d) edge (e) edge (g)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}

==> figures/dtrees/F10.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=red!50] (b) {$8$}
;}\newcommand{\nodec}{\node[draw,circle,fill=red!50] (c) {$5$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=red!50] (g) {$9$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$7$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle,fill=red!50] (j) {$4$}
;}\newcommand{\nodeba}{\node[draw,circle,fill=red!50] (ba) {$1$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$3$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$$}
;}\newcommand{\nodebe}{\node[draw,circle] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle,fill=red!50] (bh) {$6$}
;}\newcommand{\nodebi}{\node[draw,circle] (bi) {$$}
;}\newcommand{\nodebj}{\node[draw,circle,fill=red!50] (bj) {$2$}
;}\newcommand{\nodeca}{\node[draw,circle] (ca) {$$}
;}\newcommand{\nodecb}{\node[draw,circle] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle] (cc) {$$}
;}\newcommand{\nodecd}{\node[draw,circle] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \& \nodef  \&         \&         \&         \&         \& \nodeg  \&         \& \nodecd \\ 
         \& \nodec  \&         \&         \& \nodeh  \&         \&         \&         \& \nodebh \& \nodecc \&         \\ 
 \noded  \&         \& \nodee  \& \nodei  \&         \&         \& \nodej  \& \nodebi \& \nodebj \& \nodecb \&         \\ 
         \&         \&         \&         \& \nodeba \&         \& \nodebc \& \nodebg \& \nodeca \&         \&         \\ 
         \&         \&         \&         \& \nodebb \& \nodebd \& \nodebe \& \nodebf \&         \&         \&         \\
};

\path[ultra thick, red] (c) edge (d) edge (e)
	(b) edge (c)
	(ba) edge (bb)
	(bc) edge (bd) edge (be) edge (bf)
	(j) edge (ba) edge (bc) edge (bg)
	(h) edge (i) edge (j)
	(bj) edge (ca)
	(bh) edge (bi) edge (bj) edge (cb)
	(g) edge (h) edge (bh) edge (cc)
	(a) edge (b) edge (f) edge (g) edge (cd);
\end{tikzpicture}}

==> figures/dtrees/F10_2.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=white] (b) {$5$}
;}\newcommand{\nodec}{\node[draw,circle,fill=white] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle,fill=white] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle,fill=red!50] (e) {$8$}
;}\newcommand{\nodef}{\node[draw,circle,fill=red!50] (f) {$7$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle,fill=white] (i) {$9$}
;}\newcommand{\nodej}{\node[draw,circle,fill=red!50] (j) {$4$}
;}\newcommand{\nodeba}{\node[draw,circle,fill=white] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle,fill=red!50] (bb) {$3$}
;}\newcommand{\nodebc}{\node[draw,circle,fill=red!50] (bc) {$1$}
;}\newcommand{\nodebd}{\node[draw,circle,fill=white] (bd) {$$}
;}\newcommand{\nodebe}{\node[draw,circle,fill=white] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle,fill=white] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle,fill=white] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle,fill=white] (bh) {$$}
;}\newcommand{\nodebi}{\node[draw,circle,fill=red!50] (bi) {$6$}
;}\newcommand{\nodebj}{\node[draw,circle,fill=white] (bj) {$$}
;}\newcommand{\nodeca}{\node[draw,circle,fill=red!50] (ca) {$2$}
;}\newcommand{\nodecb}{\node[draw,circle,fill=white] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle,fill=white] (cc) {$$}
;}\newcommand{\nodecd}{\node[draw,circle,fill=white] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \&         \& \nodee  \&         \&         \&         \&         \& \nodei  \&         \&         \& \nodecd \\ 
 \nodec  \&         \& \noded  \&         \& \nodef  \&         \&         \& \nodej  \&         \& \nodebh \&         \& \nodebi \&         \\ 
         \&         \&         \& \nodeg  \&         \& \nodeh  \& \nodeba \& \nodebb \& \nodebg \&         \& \nodebj \& \nodeca \& \nodecc \\ 
         \&         \&         \&         \&         \&         \& \nodebc \& \nodebe \& \nodebf \&         \&         \& \nodecb \&         \\ 
         \&         \&         \&         \&         \&         \& \nodebd \&         \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(f) edge (g) edge (h)
	(e) edge (f)
	(bc) edge (bd)
	(bb) edge (bc) edge (be) edge (bf)
	(j) edge (ba) edge (bb) edge (bg)
	(ca) edge (cb)
	(bi) edge (bj) edge (ca) edge (cc)
	(i) edge (j) edge (bh) edge (bi)
	(a) edge (b) edge (e) edge (i) edge (cd);
\end{tikzpicture}}

==> figures/dtrees/F10_inter.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=white] (b) {$5$}
;}\newcommand{\nodec}{\node[draw,circle,fill=white] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle,fill=white] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle,fill=white] (e) {$8$}
;}\newcommand{\nodef}{\node[draw,circle,fill=white] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$9$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$7$}
;}\newcommand{\nodei}{\node[draw,circle,fill=white] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle,fill=red!50] (j) {$4$}
;}\newcommand{\nodeba}{\node[draw,circle,fill=white] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle,fill=white] (bb) {$3$}
;}\newcommand{\nodebc}{\node[draw,circle,fill=white] (bc) {$1$}
;}\newcommand{\nodebd}{\node[draw,circle,fill=white] (bd) {$$}
;}\newcommand{\nodebe}{\node[draw,circle,fill=white] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle,fill=white] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle,fill=white] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle,fill=white] (bh) {$$}
;}\newcommand{\nodebi}{\node[draw,circle,fill=red!50] (bi) {$6$}
;}\newcommand{\nodebj}{\node[draw,circle,fill=white] (bj) {$$}
;}\newcommand{\nodeca}{\node[draw,circle,fill=red!50] (ca) {$2$}
;}\newcommand{\nodecb}{\node[draw,circle,fill=white] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle,fill=white] (cc) {$$}
;}\newcommand{\nodecd}{\node[draw,circle,fill=white] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \& \nodee  \&         \&         \&         \& \nodeg  \&         \&         \&         \& \nodecd \\ 
 \nodec  \&         \& \noded  \& \nodef  \& \nodeh  \&         \&         \& \nodebh \&         \& \nodebi \&         \&         \\ 
         \&         \&         \& \nodei  \&         \& \nodej  \&         \&         \& \nodebj \& \nodeca \& \nodecc \&         \\ 
         \&         \&         \&         \& \nodeba \& \nodebb \& \nodebg \&         \&         \& \nodecb \&         \&         \\ 
         \&         \&         \&         \& \nodebc \& \nodebe \& \nodebf \&         \&         \&         \&         \&         \\ 
         \&         \&         \&         \& \nodebd \&         \&         \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(e) edge (f)
	(bc) edge (bd)
	(bb) edge (bc) edge (be) edge (bf)
	(j) edge (ba) edge (bb) edge (bg)
	(h) edge (i) edge (j)
	(ca) edge (cb)
	(bi) edge (bj) edge (ca) edge (cc)
	(g) edge (h) edge (bh) edge (bi)
	(a) edge (b) edge (e) edge (g) edge (cd);
\end{tikzpicture}}

==> figures/dtrees/T10_example_pure_max.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$8$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$5$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$7$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$9$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$4$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$3$}
;}\newcommand{\nodebe}{\node[draw,circle] (be) {$1$}
;}\newcommand{\nodebf}{\node[draw,circle] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle] (bh) {$$}
;}\newcommand{\nodebi}{\node[draw,circle] (bi) {$$}
;}\newcommand{\nodebj}{\node[draw,circle] (bj) {$6$}
;}\newcommand{\nodeca}{\node[draw,circle] (ca) {$$}
;}\newcommand{\nodecb}{\node[draw,circle] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle] (cc) {$2$}
;}\newcommand{\nodecd}{\node[draw,circle] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeg  \&         \&         \& \nodej  \&         \&         \&         \&         \\ 
         \&         \& \noded  \& \nodeh  \&         \& \nodei  \& \nodeba \& \nodebb \&         \&         \& \nodebj \&         \\ 
         \& \nodee  \&         \& \nodef  \&         \&         \& \nodebc \& \nodebd \& \nodebi \& \nodeca \& \nodecb \& \nodecc \\ 
         \&         \&         \&         \&         \&         \& \nodebe \& \nodebg \& \nodebh \&         \&         \& \nodecd \\ 
         \&         \&         \&         \&         \&         \& \nodebf \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e) edge (f)
	(c) edge (d)
	(g) edge (h) edge (i)
	(be) edge (bf)
	(bd) edge (be) edge (bg) edge (bh)
	(bb) edge (bc) edge (bd) edge (bi)
	(cc) edge (cd)
	(bj) edge (ca) edge (cb) edge (cc)
	(j) edge (ba) edge (bb) edge (bj)
	(a) edge (b) edge (c) edge (g) edge (j);
\end{tikzpicture}}

==> figures/dtrees/T10_example_pure_max2.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$5$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$9$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$8$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$7$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$4$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$3$}
;}\newcommand{\nodebe}{\node[draw,circle] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle] (bf) {$1$}
;}\newcommand{\nodebg}{\node[draw,circle] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle] (bh) {$$}
;}\newcommand{\nodebi}{\node[draw,circle] (bi) {$$}
;}\newcommand{\nodebj}{\node[draw,circle] (bj) {$6$}
;}\newcommand{\nodeca}{\node[draw,circle] (ca) {$$}
;}\newcommand{\nodecb}{\node[draw,circle] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle] (cc) {$2$}
;}\newcommand{\nodecd}{\node[draw,circle] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \& \nodee  \&         \&         \&         \& \nodef  \&         \&         \& \nodebj \&         \\ 
 \nodec  \&         \& \noded  \&         \& \nodeg  \&         \&         \& \nodeba \& \nodebi \& \nodeca \& \nodecb \& \nodecc \\ 
         \&         \&         \&         \& \nodeh  \&         \& \nodebb \& \nodebc \& \nodebd \&         \&         \& \nodecd \\ 
         \&         \&         \& \nodei  \&         \& \nodej  \&         \& \nodebe \& \nodebf \& \nodebh \&         \&         \\ 
         \&         \&         \&         \&         \&         \&         \&         \& \nodebg \&         \&         \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(h) edge (i) edge (j)
	(g) edge (h)
	(bf) edge (bg)
	(bd) edge (be) edge (bf) edge (bh)
	(ba) edge (bb) edge (bc) edge (bd)
	(f) edge (g) edge (ba) edge (bi)
	(cc) edge (cd)
	(bj) edge (ca) edge (cb) edge (cc)
	(a) edge (b) edge (e) edge (f) edge (bj);
\end{tikzpicture}}

==> figures/dtrees/T10_example_pure_max_inter.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$5$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$8$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$9$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$7$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$4$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$3$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$1$}
;}\newcommand{\nodebe}{\node[draw,circle] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle] (bh) {$$}
;}\newcommand{\nodebi}{\node[draw,circle] (bi) {$$}
;}\newcommand{\nodebj}{\node[draw,circle] (bj) {$6$}
;}\newcommand{\nodeca}{\node[draw,circle] (ca) {$$}
;}\newcommand{\nodecb}{\node[draw,circle] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle] (cc) {$2$}
;}\newcommand{\nodecd}{\node[draw,circle] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \& \nodee  \&         \&         \&         \& \nodeg  \&         \&         \& \nodebj \&         \\ 
 \nodec  \&         \& \noded  \& \nodef  \& \nodeh  \&         \&         \& \nodeba \& \nodebi \& \nodeca \& \nodecb \& \nodecc \\ 
         \&         \&         \& \nodei  \&         \& \nodej  \& \nodebb \& \nodebc \& \nodebh \&         \&         \& \nodecd \\ 
         \&         \&         \&         \&         \&         \& \nodebd \& \nodebf \& \nodebg \&         \&         \&         \\ 
         \&         \&         \&         \&         \&         \& \nodebe \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(e) edge (f)
	(h) edge (i) edge (j)
	(bd) edge (be)
	(bc) edge (bd) edge (bf) edge (bg)
	(ba) edge (bb) edge (bc) edge (bh)
	(g) edge (h) edge (ba) edge (bi)
	(cc) edge (cd)
	(bj) edge (ca) edge (cb) edge (cc)
	(a) edge (b) edge (e) edge (g) edge (bj);
\end{tikzpicture}}

==> figures/dtrees/T10_example_pure_min.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$10$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$8$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$5$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$9$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$7$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$4$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$1$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$3$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$$}
;}\newcommand{\nodebe}{\node[draw,circle] (be) {$$}
;}\newcommand{\nodebf}{\node[draw,circle] (bf) {$$}
;}\newcommand{\nodebg}{\node[draw,circle] (bg) {$$}
;}\newcommand{\nodebh}{\node[draw,circle] (bh) {$6$}
;}\newcommand{\nodebi}{\node[draw,circle] (bi) {$$}
;}\newcommand{\nodebj}{\node[draw,circle] (bj) {$2$}
;}\newcommand{\nodeca}{\node[draw,circle] (ca) {$$}
;}\newcommand{\nodecb}{\node[draw,circle] (cb) {$$}
;}\newcommand{\nodecc}{\node[draw,circle] (cc) {$$}
;}\newcommand{\nodecd}{\node[draw,circle] (cd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \&         \&         \&         \&         \&         \&         \\ 
         \& \nodeb  \&         \& \nodef  \&         \&         \&         \&         \&         \& \nodeg  \&         \&         \& \nodecd \\ 
         \& \nodec  \&         \&         \& \nodeh  \&         \&         \&         \&         \& \nodebh \&         \& \nodecc \&         \\ 
 \noded  \&         \& \nodee  \& \nodei  \&         \&         \& \nodej  \&         \& \nodebi \& \nodebj \& \nodecb \&         \&         \\ 
         \&         \&         \&         \& \nodeba \&         \& \nodebc \& \nodebg \&         \& \nodeca \&         \&         \&         \\ 
         \&         \&         \&         \& \nodebb \& \nodebd \& \nodebe \& \nodebf \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (c) edge (d) edge (e)
	(b) edge (c)
	(ba) edge (bb)
	(bc) edge (bd) edge (be) edge (bf)
	(j) edge (ba) edge (bc) edge (bg)
	(h) edge (i) edge (j)
	(bj) edge (ca)
	(bh) edge (bi) edge (bj) edge (cb)
	(g) edge (h) edge (bh) edge (cc)
	(a) edge (b) edge (f) edge (g) edge (cd);
\end{tikzpicture}}

==> figures/dtrees/T5_notpure1.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$5$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$4$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$3$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$2$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$1$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \&         \& \nodea  \&         \\ 
         \&         \&         \& \nodeb  \&         \& \nodeba \& \nodebb \\ 
         \& \nodec  \&         \& \nodei  \& \nodej  \&         \&         \\ 
 \noded  \& \nodef  \& \nodeh  \&         \&         \&         \&         \\ 
 \nodee  \& \nodeg  \&         \&         \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(f) edge (g)
	(c) edge (d) edge (f) edge (h)
	(b) edge (c) edge (i) edge (j)
	(a) edge (b) edge (ba) edge (bb);
\end{tikzpicture}}

==> figures/dtrees/T5_notpure2.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$5$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$4$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$3$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$1$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \&         \&         \& \noded  \&         \& \nodebb \\ 
 \nodec  \&         \& \nodee  \&         \& \nodei  \& \nodeba \&         \\ 
         \& \nodef  \& \nodeg  \& \nodeh  \& \nodej  \&         \&         \\
};

\path[ultra thick, red] (b) edge (c)
	(e) edge (f) edge (g) edge (h)
	(i) edge (j)
	(d) edge (e) edge (i) edge (ba)
	(a) edge (b) edge (d) edge (bb);
\end{tikzpicture}}

==> figures/dtrees/T6_stamari.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$6$}
;}\newcommand{\nodeb}{\node[draw,circle, ,fill=red!50] (b) {$4$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$1$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$2$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$3$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$5$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \&         \&         \&         \&         \& \nodea  \&         \&         \\ 
         \&         \& \nodeb  \&         \&         \&         \&         \&         \& \nodeba \&         \& \nodebd \\ 
 \nodec  \&         \& \nodee  \&         \&         \& \nodeh  \&         \& \nodebb \&         \& \nodebc \&         \\ 
 \noded  \& \nodef  \&         \& \nodeg  \& \nodei  \&         \& \nodej  \&         \&         \&         \&         \\
};

\path[ultra thick, red] (c) edge (d)
	(e) edge (f) edge (g)
	(h) edge (i) edge (j)
	(b) edge (c) edge (e) edge (h)
	(ba) edge (bb) edge (bc)
	(a) edge (b) edge (ba) edge (bd);
\end{tikzpicture}}


==> figures/dtrees/T6_stamari2.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$6$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$1$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$5$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$4$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$2$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle] (j) {$3$}
;}\newcommand{\nodeba}{\node[draw,circle] (ba) {$$}
;}\newcommand{\nodebb}{\node[draw,circle] (bb) {$$}
;}\newcommand{\nodebc}{\node[draw,circle] (bc) {$$}
;}\newcommand{\nodebd}{\node[draw,circle] (bd) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \&         \&         \&         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \&         \&         \&         \&         \&         \&         \& \noded  \&         \& \nodebd \\ 
 \nodec  \&         \&         \& \nodee  \&         \&         \&         \&         \&         \& \nodebc \&         \\ 
         \& \nodef  \&         \& \nodeg  \&         \&         \& \nodej  \&         \&         \&         \&         \\ 
         \&         \& \nodeh  \&         \& \nodei  \& \nodeba \&         \& \nodebb \&         \&         \&         \\
};

\path[ultra thick, red] (b) edge (c)
	(g) edge (h) edge (i)
	(j) edge (ba) edge (bb)
	(e) edge (f) edge (g) edge (j)
	(d) edge (e) edge (bc)
	(a) edge (b) edge (d) edge (bd);
\end{tikzpicture}}

==> figures/dtrees/T_012_two_facets1.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$1$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$2$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \noded  \&         \& \nodeg  \\ 
 \nodec  \& \nodee  \&         \& \nodef  \&         \\
};

\path[ultra thick, red] (b) edge (c)
	(d) edge (e) edge (f)
	(a) edge (b) edge (d) edge (g);
\end{tikzpicture}}

==> figures/dtrees/T_012_two_facets2.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$1$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeg  \\ 
         \& \noded  \&         \& \nodef  \&         \\ 
         \& \nodee  \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(c) edge (d) edge (f)
	(a) edge (b) edge (c) edge (g);
\end{tikzpicture}}

==> figures/dtrees/T_012_two_facets3.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$1$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$2$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \& \nodea  \&         \&         \&         \\ 
 \nodeb  \& \noded  \&         \& \nodee  \&         \\ 
 \nodec  \&         \& \nodef  \&         \& \nodeg  \\
};

\path[ultra thick, red] (b) edge (c)
	(e) edge (f) edge (g)
	(a) edge (b) edge (d) edge (e);
\end{tikzpicture}}

==> figures/dtrees/T_012_two_facets4.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$1$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$2$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \& \nodea  \&         \&         \&         \\ 
 \nodeb  \& \nodec  \&         \& \nodee  \&         \\ 
         \& \noded  \& \nodef  \&         \& \nodeg  \\
};

\path[ultra thick, red] (c) edge (d)
	(e) edge (f) edge (g)
	(a) edge (b) edge (c) edge (e);
\end{tikzpicture}}


==> figures/dtrees/T_012_two_facets5.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$1$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodef  \& \nodeg  \\ 
 \nodec  \&         \& \nodee  \&         \&         \\ 
 \noded  \&         \&         \&         \&         \\
};

\path[ultra thick, red] (c) edge (d)
	(b) edge (c) edge (e)
	(a) edge (b) edge (f) edge (g);
\end{tikzpicture}}

==> figures/dtrees/T_012_two_facets6.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$1$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodef  \& \nodeg  \\ 
 \nodec  \&         \& \noded  \&         \&         \\ 
         \&         \& \nodee  \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(b) edge (c) edge (d)
	(a) edge (b) edge (f) edge (g);
\end{tikzpicture}}

==> figures/dtrees/T_012_two_facets7.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodee  \& \nodeg  \\ 
 \nodec  \&         \& \noded  \& \nodef  \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d)
	(e) edge (f)
	(a) edge (b) edge (e) edge (g);
\end{tikzpicture}}

==> figures/dtrees/T_012_two_facets8.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeg  \\ 
         \& \noded  \&         \& \nodee  \&         \\ 
         \&         \&         \& \nodef  \&         \\
};

\path[ultra thick, red] (e) edge (f)
	(c) edge (d) edge (e)
	(a) edge (b) edge (c) edge (g);
\end{tikzpicture}}

==> figures/dtrees/T_022_two_facets1.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$1$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodeg  \& \nodeh  \\ 
 \nodec  \& \nodee  \& \nodef  \&         \&         \\ 
 \noded  \&         \&         \&         \&         \\
};

\path[ultra thick, red] (c) edge (d)
	(b) edge (c) edge (e) edge (f)
	(a) edge (b) edge (g) edge (h);
\end{tikzpicture}}

==> figures/dtrees/T_022_two_facets2.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$1$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$2$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \noded  \&         \& \nodeh  \\ 
 \nodec  \& \nodee  \& \nodef  \& \nodeg  \&         \\
};

\path[ultra thick, red] (b) edge (c)
	(d) edge (e) edge (f) edge (g)
	(a) edge (b) edge (d) edge (h);
\end{tikzpicture}}

==> figures/dtrees/T_022_two_facets3.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$1$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodef  \& \nodeg  \&         \\ 
         \& \nodee  \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(c) edge (d) edge (f) edge (g)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}


==> figures/dtrees/T_022_two_facets4.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$1$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodeg  \& \nodeh  \\ 
 \nodec  \& \noded  \& \nodef  \&         \&         \\ 
         \& \nodee  \&         \&         \&         \\
};

\path[ultra thick, red] (d) edge (e)
	(b) edge (c) edge (d) edge (f)
	(a) edge (b) edge (g) edge (h);
\end{tikzpicture}}


==> figures/dtrees/T_022_two_facets5.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodee  \& \nodeg  \&         \\ 
         \&         \& \nodef  \&         \&         \\
};

\path[ultra thick, red] (e) edge (f)
	(c) edge (d) edge (e) edge (g)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}

==> figures/dtrees/T_022_two_facets6.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$1$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodeg  \& \nodeh  \\ 
 \nodec  \& \noded  \& \nodee  \&         \&         \\ 
         \&         \& \nodef  \&         \&         \\
};

\path[ultra thick, red] (e) edge (f)
	(b) edge (c) edge (d) edge (e)
	(a) edge (b) edge (g) edge (h);
\end{tikzpicture}}

==> figures/dtrees/T_022_two_facets7.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$2$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$1$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \& \nodea  \&         \\ 
         \& \nodeb  \&         \& \nodef  \& \nodeh  \\ 
 \nodec  \& \noded  \& \nodee  \& \nodeg  \&         \\
};

\path[ultra thick, red] (b) edge (c) edge (d) edge (e)
	(f) edge (g)
	(a) edge (b) edge (f) edge (h);
\end{tikzpicture}}

==> figures/dtrees/T_022_two_facets8.tex <==
{ \newcommand{\nodea}{\node[draw,circle] (a) {$3$}
;}\newcommand{\nodeb}{\node[draw,circle] (b) {$$}
;}\newcommand{\nodec}{\node[draw,circle] (c) {$2$}
;}\newcommand{\noded}{\node[draw,circle] (d) {$$}
;}\newcommand{\nodee}{\node[draw,circle] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle] (f) {$1$}
;}\newcommand{\nodeg}{\node[draw,circle] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle] (h) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=.3cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \& \nodea  \&         \&         \\ 
 \nodeb  \&         \& \nodec  \&         \& \nodeh  \\ 
         \& \noded  \& \nodee  \& \nodef  \&         \\ 
         \&         \&         \& \nodeg  \&         \\
};

\path[ultra thick, red] (f) edge (g)
	(c) edge (d) edge (e) edge (f)
	(a) edge (b) edge (c) edge (h);
\end{tikzpicture}}

==> figures/pure_face.tex <==
{ \newcommand{\nodea}{\node[draw,circle,fill=white] (a) {$4$}
;}\newcommand{\nodeb}{\node[draw,circle,fill=red!50] (b) {$3$}
;}\newcommand{\nodec}{\node[draw,circle,fill=white] (c) {$$}
;}\newcommand{\noded}{\node[draw,circle,fill=red!50] (d) {$2$}
;}\newcommand{\nodee}{\node[draw,circle,fill=white] (e) {$$}
;}\newcommand{\nodef}{\node[draw,circle,fill=white] (f) {$1$}
;}\newcommand{\nodeg}{\node[draw,circle,fill=white] (g) {$$}
;}\newcommand{\nodeh}{\node[draw,circle,fill=white] (h) {$$}
;}\newcommand{\nodei}{\node[draw,circle,fill=white] (i) {$$}
;}\newcommand{\nodej}{\node[draw,circle,fill=white] (j) {$$}
;}\begin{tikzpicture}[auto]
\matrix[column sep=0.1cm, row sep=.3cm,ampersand replacement=\&]{
         \&         \&         \&         \&         \& \nodea  \&         \\ 
         \&         \& \nodeb  \&         \&         \&         \& \nodej  \\ 
 \nodec  \&         \& \noded  \&         \& \nodei  \&         \&         \\ 
         \& \nodee  \& \nodef  \& \nodeh  \&         \&         \&         \\ 
         \&         \& \nodeg  \&         \&         \&         \&         \\
};

\path[ultra thick, red] (f) edge (g)
	(d) edge (e) edge (f) edge (h)
	(b) edge (c) edge (d) edge (i)
	(a) edge (b) edge (j);
\end{tikzpicture}}

==> figures/pure_intersection.tex <==
\begin{tabular}{ccc}
\scalebox{.6}{\input{figures/dtrees/F10}} & 
\scalebox{.6}{\input{figures/dtrees/T10_example_pure_max}} \\
\scalebox{.6}{\input{figures/dtrees/F10_2}} & 
\scalebox{.6}{\input{figures/dtrees/T10_example_pure_max2}} \\ \hline
Intersection & \\
\scalebox{.6}{\input{figures/dtrees/F10_inter}} & 
\scalebox{.6}{\input{figures/dtrees/T10_example_pure_max_inter}}
\end{tabular}
